Accessibility of Nilpotent Orbits in Classical Algebras

Let $G$ be a classical linear algebraic group over an algebraically closed field, and let $\mathfrak{n}$ denote the subset of nilpotent elements in its Lie algebra. In this paper we study a partial order on the $G$-orbits in $\mathfrak{n}$ given by taking limits along cocharacters of $G$. This gives rise to the so-called accessibility order on the nilpotent orbits. Our main results show that for general and special linear algebras, this new order coincides with the usual dominance order on nilpotent orbits, but for symplectic and orthogonal algebras this is not the case.

==> ANOA_Results_OtherClassical.tex <==
\section{Results in other classical groups}
\subsection{The symplectic algebras}
First, recall the possible $\mathfrak{sp}_{2n}$-partitions, and which orbits are distinguished. The symplectic partitions are given by the theorem \textcolor{red}{(Refer to theorem in introduction)}:
\begin{theorem}
	Let $x$ be a nilpotent element with partition $[r_1^{(n_1)},\ldots,r_p^{(n_p)}]$. Then $x$ appears in $\mathfrak{sp}_{2n}$ if and only if $n_i$ is even for all odd $r_i$.
\end{theorem}
And the Lemma \textcolor{red}{Refer to Lemma in introduction} tells when orbits are distinguished:
\begin{lemma}
	Let $x\in \mathfrak{sp}_{2n}$, then $x$ is distinguished if and only if its partition $\pi$ has distinct even parts (and no odd parts).
\end{lemma}
By considering minimal moves through the dominance order of the partitions corresponding to the orbits, the following moves are identified, and $m=0$ can occur:
\begin{enumerate}
	\item $\mathcal{O}([2m,2m-2])		\rightarrow \mathcal{O}([2m-1,2m-1])$.
	\item $\mathcal{O}([2n,m,m])		\rightarrow \mathcal{O}([2n-2,m+1,m+1])$.
	\item $\mathcal{O}([n,n,2m])		\rightarrow \mathcal{O}([n-1,n-1,2m+2])$.
	\item $\mathcal{O}([n,n,m,m])		\rightarrow \mathcal{O}([n-1,n-1,m+1,m+1])$.
	\item $\mathcal{O}([2n,2m])			\rightarrow \mathcal{O}([2n-2,2m+2])$.
\end{enumerate}
Section \textcolor{red}{Reference to correct section} shows that move 5 does not occur, which is obvious if $m=0$, since then the target orbit is distinguished. In the following section, examples of moves 1-4 will be given.
\subsection{Cocharacters realising moves 1-4}\label{SympPartitionsMoves}
For each of the moves, matrices $x$ and $x'$ will be given, and the starting vectors of the vector seqences that $x'$ induces. Then, the $\lambda$ to obtain $y=\lim_\lambda x'$ will be given.

\emph{Move 1: $\mathcal{O}([2m,2m-2])		\rightarrow \mathcal{O}([2m-1,2m-1])$.} Let:
$$x=\left(\begin{array}{ccc|ccc|cc}
	&  &  &  &  &  &  &    \\ 
	& J_{m} &  &  &  &  &  &    \\ 
	&  &  &  &  &  & 1_{(a)} &    \\ 
	\hline
	&  &  &  &  &  &  &    \\ 
	&  &  &  & \tilde{J}_{2m-2} &  &  &    \\ 
	&  &  &  &  &  &  &    \\ 
	\hline
	&  &  &  &  &  &  &    \\ 
	&  &  &  &  &  & -J_{m} &    \\ 
	&  &  &  &  &  &  &   
\end{array}\right),x'=\left(\begin{array}{ccc|ccc}
	&  &  & 1_{(b)} &  &  \\ 
	& J_{2m-1} &  &  &  &  \\ 
	&  &  &  &  & \!\!\!\!\!\!1_{(c)} \\ 
	\hline
	&  &  &  &  &  \\ 
	&  &  &  & \!\!\!\!\!\!\!\!\!\!-J_{2m-1} &  \\ 
	&  &  &  &  & 
\end{array}\right),$$
with $(a)=(m,3m-1)$, $(b)=(1,2m)$ and $(c)=(2m-1,4m-2)$.
Then $x'$ induces a vector sequence of size $2m$ (starting in $f_1$) and a vector sequence of size $2m-2$ (starting in $f_2-e_n$), hence it is in the orbit $\mathcal{O}([2m,2m-2])$. Taking $\lambda=\text{diag}(tI_{2m-1},t^{-1}I_{2m-1})$ yields $y=\lim_\lambda x'\in \mathcal{O}([2m-1,2m-1])$, hence $\mathcal{O}([2m-1,2m-1])$ is 1-accessible from $\mathcal{O}([2m,2m-2])$.

\emph{Move 2: $\mathcal{O}([2n,m,m])		\rightarrow \mathcal{O}([2n-2,m+1,m+1])$.} Let $x=J_m \oplus\tilde{J}_{2n}\oplus (-J_m)$ \textcolor{red}{Explain what $\tilde{J}_{2n}$ means} and let

$$x'=\left(\begin{array}{ccc|ccc|cc}
	&  &  & 1_{(a)} &  &  &  &   \\ 
	& J_{m+1} &  &  &  &  &  &    \\ 
	&  &  &  &  &  &  &    \\ 
	\hline
	&  &  &  &  &  &  &    \\ 
	&  &  &  & \tilde{J}_{2n-2} &  &  &    \\ 
	&  &  &  &  &  &  & -1_{(b)}   \\ 
	\hline
	&  &  &  &  &  &  &    \\ 
	&  &  &  &  &  & -J_{m+1} &    \\ 
	&  &  &  &  &  &  &   
\end{array}\right),$$
with $(a)=(1,m+2)$ and $b=(m+2n-1,2m+2n)$. Then $x'$ induces three vector sequences, of size $2n$ (starting in $f_1$), $m$ (starting in $f_2$), and $m$ (starting in $e_n-e_{n+m}$). So $x\in \mathcal{O}([2n,m,m])$. Taking $\lambda=\text{diag}(tI_{m+1},I_{2n-2},t^{-1}I_{m+1})$ yields $y=\lim_\lambda x' \in \mathcal{O}([2n-2,m+1,m+1])$, so this orbit is 1-accessible from $\mathcal{O}([2n,m,m])$.

\emph{Move 3:} $\mathcal{O}([n,n,2m])		\rightarrow \mathcal{O}([n-1,n-1,2m+2]).$ Let $x=J_n \oplus \tilde{J}_{2m} \oplus (-J_n),$ and let

$$
x'=\left(\begin{array}{ccc|ccc|cc}
	&  &  &  &  &  &  &  \\ 
	& J_{n-1} &  &  &  &  &  &  \\ 
	&  &  &  &  & \!\!\!\!\!\!\!\!\!1_{(a)} &  &  \\ 
	\hline
	&  &  &  &  &  & 1_{(b)} &  \\ 
	&  &  &  & \;\; \tilde{J}_{2m+2} &  &  &  \\ 
	&  &  &  &  &  &  &  \\ 
	\hline
	&  &  &  &  &  &  &  \\ 
	&  &  &  &  &  & \;\; -J_{n-1} &  \\ 
	&  &  &  &  &  &  & 
\end{array}\right),$$
with $(a)=(n-1,n+2m+1)$ and $(b)=(n,n+2m+2)$. Then $x'$ induces three vector sequences, two of size $n$ (starting in $f_1$, and in $f_n$), and one of size $2m$ (starting in $f_{n+1}+f_{n-2m}$). So $x\in \mathcal{O}([n,n,2m])$. Taking $\lambda=\text{diag}(tI_{n-1},I_{2m+2},t^{-1}I_{n-1})$ yields $y=\lim_\lambda x'\in \mathcal{O}([n-1,n-1,2m+2])$, so this orbit is 1-accessible from $\mathcal{O}([n,n,2m])$.

\emph{Move 4:$\mathcal{O}([n,n,m,m])		\rightarrow \mathcal{O}([n-1,n-1,m+1,m+1])$.} Let $x=J_m\oplus J_n \oplus (-J_n) \oplus (-J_m),$, and let $$x'=\left(\begin{array}{ccc|ccc|ccc|ccc}
	&  &  & 1_{(a)} &  &  &  &  &  &  &  &  \\ 
	& J_{m+1} &  &  &  &  &  &  &  &  &  &  \\ 
	&  &  &  &  &  &  &  &  &  &  &  \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  \\ 
	&  &  &  & J_{n-1} &  &  &  &  &  &  &  \\ 
	&  &  &  &  &  &  &  &  &  &  &  \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  \\ 
	&  &  &  &  &  &  & -J_{n-1} &  &  &  &  \\ 
	&  &  &  &  &  &  &  &  &  &  & 1_{(b)} \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  \\ 
	&  &  &  &  &  &  &  &  &  & -J_{m+1} &  \\ 
	&  &  &  &  &  &  &  &  &  &  & 
\end{array} \right),$$
with $(a)=(1,m+2)$ and $(b)=(m+2n-1,2m+2n).$ Then $x'$ induces four vector sequences, two of size $n$ (starting in $f_1$ and $e_{n+m}$, respectively) and two of size $m$ (starting in $f_2$ and $e_{1+m}-e_{1+2m}$, respectively). So $x\in \mathcal{O}([n,n,m,m])$. Taking $\lambda=\text{diag}(t^2I_{m+1},tI_{n-1},t^{-1}I_{n-1},t^{-2}I_{m+1})$ yields $y=\lim_\lambda x'\in \mathcal{O}([n-1,n-1,m+1,m+1])$, so this orbit is 1-accessible from $\mathcal{O}([n,n,m,m])$.

\subsection{A non-move}\label{Subsec:NonMove}
This section will analyse Move 5: $\mathcal{O}([2n,2m])\rightarrow \mathcal{O}([2n-2,2m+2])$, starting with examples in Section \ref{Subsec:NonMoveExamples}, followed by the set-up of the requirements of the nonmove, and finally the proof itself.

\subsubsection{Examples}\label{Subsec:NonMoveExamples}First, consider that if $2n-2=2m+2$, then this move is actually a generalized move 1, of the form $\mathcal{O}([2m,2m-2k])\rightarrow \mathcal{O}([2m-k,2m-k])$, with $k=2$. So for move 5, the case where $2n-2\neq 2m+2$ is considered.

Starting with an example, consider the move $\mathcal{O}([6])\rightarrow \mathcal{O}([4,2])$ (so $m=0$) From Lemma \ref{Lem:CentralLambda}, one can see that the target orbit is distinguished, so it is not accessible from the starting orbit. However, it is still worth calculating directly, so let $x\in \mathcal{O}([6])$ be in standard form:
$$x=\left(\begin{array}{cccccc}
	0 & 1 & 0 & 0 & 0 & 0 \\ 
	0 & 0 & 1 & 0 & 0 & 0 \\ 
	0 & 0 & 0 & 1 & 0 & 0 \\ 
	0 & 0 & 0 & 0 & -1 & 0 \\ 
	0 & 0 & 0 & 0 & 0 & -1 \\ 
	0 & 0 & 0 & 0 & 0 & 0
\end{array}\right).$$
Next, a matrix $x'$ has to be determined, such that $y=\lim_{\lambda}x'\in \mathcal{O}([4,2])$ for a suitable $\lambda$. Then $\lambda$ has to be in the centralizer of $y$, so the forms of $y$ and $\lambda$ will be determined first:
$$y=\left(\begin{array}{cccccc}
	0 & 0 & 0 & 0 & 0 & 1 \\ 
	0 & 0 & 1 & 0 & 0 & 0 \\ 
	0 & 0 & 0 & 1 & 0 & 0 \\ 
	0 & 0 & 0 & 0 & -1 & 0 \\ 
	0 & 0 & 0 & 0 & 0 & 0 \\ 
	0 & 0 & 0 & 0 & 0 & 0
\end{array}\right),$$
and $\lambda=\text{diag}(t_1,t_2,t_3,t_4,t_5,t_6).$ As $\lim_{\lambda}x'=y$, the restriction is that
$$\lim_{t\rightarrow 0} t_1x'_{( 1,6)}t_6^{-1} = 1,$$
so $t_1=t_6$, hence all $t_i$ must be equal. The only $\lambda$ in $\text{Stab}_G(y)$ is $\pm I$, which is in the centre of $y$. Hence $x'=y$, and $y$ is not accessible from $x$. This is a special case of a general phenomenom: if the target element $y$ is distinguished, then there cannot be any non-trivial cocharacter with $\lim_\lambda x' = y$.
\textcolor{red}{Now the second example}
Now that it is shown that $\mathcal{O}([2n,2m])\rightarrow \mathcal{O}([2n-2,2m+2])$ is not a valid move if $2n-2\neq 2m+2$, one can consider the implications to the general accessibility of orbits. The following diagram is the diagram of 1-accessibility in $\mathfrak{sp}_6$, to compare to the diagram for $\mathfrak{gl}_6$ (see Figure \ref{fig:DominanceGL6} \textcolor{red}{Reference the dominance figure for $\mathfrak{gl}_6$}).

\textcolor{red}{Tikzpicture doesn't work}

The observation that $\mathcal{O}([4,2])$ is not accessible from $\mathcal{O}([6])$ gives an answer to the second question in \ref{enum:questions}: When $\kappa=\overline{\kappa}$, are there cases when $\overline{G(\kappa)\cdot x}^c\neq \overline{G(\kappa)\cdot x}$? Yes, as $\mathcal{O}([4,2])$ is not in the cocharacter-closure of $\mathcal{O}([6])$. 
In general, however, this observation does not give the complete answer, since the presence of other parts in the partition can complicate matters. For example, even though $\mathcal{O}([4,2])$ is not accessible from $\mathcal{O}([6])$, we can show that $\mathcal{O}([4,2,2])$ is 1-accessible from $\mathcal{O}([6,2])$. The presence of the extra part of size 2 in the partition makes a material difference to the outcome, which is not obvious immediately. Note in this case that the two partitions are no longer adjacent in the dominance order -- the accessibility diagram for this case can be split as follows: \textcolor{red}{tikzpicture doesn't work}

Consecutively applying move 1 to the $[2]$ part of $[6,2]$ ($[2m,2m-2]\rightarrow [2m-1,2m-1]$ for $m=1$) and move 2 to the partition $[6,1,1]$ ($[2n,m,m] \rightarrow [2n-2,m+1,m+1]$ for $n=3$, $m=1$), shows that $\mathcal{O}([4,2,2])$ is accessible from $\mathcal{O}([6,2])$. Proving 1-accessibility for these orbits is left to the reader. With these examples in mind, a precise analysis of move 5 follows in the next section. \textcolor{red}{Actually, setup first}

\subsubsection{The Shrinking Operation}\label{Subsec:ShrinkOp}
To prove that move 5 does not occur, a new operation will be introduced. Define the shrinking operation as follows: given a $2n \times 2n$ matrix $A$, matrix $S(A)$ is the $(2n-2) \times (2n-2)$ matrix formed by deleting rows and columns on the outside of matrix $A$. For example, let:

$$A=\left(\begin{array}{cccc}
	a_{(1,1)} & a_{(1,2)} & a_{(1,3)} & a_{(1,4)} \\ 
	a_{(2,1)} & a_{(2,2)} & a_{(2,3)} & a_{(2,4)} \\ 
	a_{(3,1)} & a_{(3,2)} & a_{(3,3)} & a_{(3,4)} \\ 
	a_{(4,1)} & a_{(4,2)} & a_{(4,3)} & a_{(4,4)}
\end{array}\right), \text{ then }
S(A)=\left(\begin{array}{cc}
	a_{(2,2)} & a_{(2,3)} \\ 
	a_{(3,2)} & a_{(3,3)}
\end{array}\right).$$
Denote by $S^d(A)$ the $(2n-2d)\times (2n-2d)$ matrix formed repeating the shrinking operation $d$ times. The shrinking operation is well-behaved with respect to the transpose $S^d(A^T)=(S^d(A))^T$. To show that $S$ is also well-behaved with respect to being in the symplectic Lie algebra, observe that when $\Omega_\text{S}$ is the defining matrix for the form in dimension $2n$, then $S^d(\Omega_\text{S})$ is the defining matrix in dimension $2n-2d$. Then if $A^T\Omega_\text{S}+\Omega_\text{S} A=0,$ it follows that $S^d(A^T)S^d(\Omega_\text{S})+S^d(\Omega_\text{S})S^d(A)=0$. 

Next, suppose $y$ is  in standard form and $\dim(y)=2n$. If $x$ is such that $\lim_{\lambda}x=y$ and $\lambda$ is in standard form (as in \ref{sec:ToriCochar}, then $\lim_{S^d(\lambda)}S^d(x)=S^d(y)$. There are now two possibilities:
\begin{enumerate}
	\item $S^d(x)$ is conjugate to $S^d(y)$, i.e. no orbit change is made.
	\item $S^d(x)$ is strictly higher than $S^d(y)$ in the dominance order.
\end{enumerate}
With these observations in hand, further reductions can be made.
\subsubsection{The setup}\label{Subsec:setup}
It has already been shown that distinguished partitions are not accessible from any partition higher in the dominance order. The question is: are non-distinguished partitions accessible through a `move' of type 5? This is the case of interest, so the following assumptions can be made:

\begin{enumerate}
	\item[(i)] $y$ is in standard form with a repeated part $[\ldots,d,d,\ldots]$ appearing on the outside of $y$ (so $y$ is not distinguished).
	\item[(ii)] $x$ is another nilpotent element.
	\item[(iii)] $\lambda$ is a cocharacter in standard form such that $\lim_{\lambda} x=y$.
\end{enumerate}

Under these hypotheses, $x$ can be denoted as $x=y+x_0$, with $\lim_{\lambda} x_0 = 0$. Since $\lambda$ is in standard form, $x_0$ is strictly upper triangular. Furthermore, $\lambda$ must centralize $y$, so $\lambda$ has constant weight $a$ on the first $d$ basis vectors, and constant weight $-a$ on the last $d$ vectors, i.e. for $1\leq i \leq d$, one gets $\lambda(t)e_i=t^ae_i$, $\lambda(t)f_i=t^{-a}f_i$. Let $\lambda_0$ be the cocharacter formed by having weight $a$ on the first $d$ vectors, $-a$ on the last $d$ vectors, and weight zero elsewhere. Then $\lambda_0$ and $\lambda$ are identical on the outside $d$ vectors, and $\lambda_0$ fixes the other vectors.

Then $\lim_{\lambda_0}y=y$ and $x':=\lim_{\lambda_0}x$ exists. Since $\lim_{\lambda}x=y$, $\lim_{\lambda}x'=y$ also, hence $x'$ lies between $x$ and $y$ in the order of dominance. Hence, if $x$ and $y$ are adjacent in the order, there are two possibilities:

\begin{enumerate}
	\item $x'=y$,
	\item $x'$ is conjugate to $x$.
\end{enumerate}

In the case that $x'=y$, the only difference between $x$ and $y$ lies in the outside $d$ rows and columns, i.e. $S^d(x)=S^d(y)$. In the case that $x'$ is conjugate with $x$, one may replace $x$ with $x'$ and assume $x$ has the same repeated $[d,d]$ blocks as $y$ on the outside. The following section will prove that both cases lead to a contradiction, hence move 5 cannot occur in a partition change between adjacent parts.

\subsubsection{The move of type 5}
The previous subsection set up the requirements to analyse move 5, does not occur, by proving the following lemma.
\begin{lemma}\label{lem:Move5Symplectic}
	Let $x\in \mathcal{O}([\ldots,2r,2s,\ldots])$ and let $y \in \mathcal{O}([\ldots,2r-2,2s+2,\ldots])$. Then $y$ is not accessible from $x$.
\end{lemma}

\begin{proof}\label{prf:NonMove}Proceed by induction on $n$, where $2n$ is the matrix size. If $n=1$, there are no $r,s$ with $2r\geq 6$. For the inductive step, suppose that for all matrix sizes smaller than $2n$ the claim holds, the following proof is a combination of contradiction and some direct calculation.
	
Suppose there is a $\lambda\in Y(G)$ such that $\lim_{\lambda}x=y$. First note that $y$ is not distinguished, by Lemma \ref{Lem:CentralLambda}. So $y$ must contain a repeated part $[\ldots,d,d,\ldots]$. With the assumption that $y$ and $\lambda$ are in standard form, one may assume that this repeated part appears on the outside of the matrix for $y$, so Section \ref{Subsec:setup} can be used. Since $x$ and $y$ are adjacent, the two cases of that section apply. Starting with the second case, suppose that $x'$ is conjugate to $x$, then $x$ and $y$ share the repeated $[\ldots,d,d\ldots]$ part. With a suitable conjugation, the repeated $d-$parts in $x$ are on the outside as well. Then the shrinking operation applied $d$ times removes that part from both $x$ and $y$. The move between $S^d(x)$ and $S^d(y)$ is of the same form as the move between $x$ and $y$, i.e. it consists of the move $[\ldots, 2r, 2s, \ldots]$ to $[\ldots,2r-2,2s+2,\ldots]$ between adjacent parts, with $2r \geq 2s+6$. Since the matrix sizes have been decreased, this is impossible, by induction. A contradiction follows, hence the second case cannot occur.

Hence case 1 of Section \ref{Subsec:setup} is left. Replacing $x$ with $x'$ and $\lambda$ with $\lambda_0$, one has that $S^d(x)=S^d(y)$ in this case \textcolor{red}{Maybe matrices here}. Note that the first $d$ rows and last $d$ columns of $x$ are related because $x$ is symplectic; if there is an entry $a$ in position $(i,j)$ then $x$ also has an entry $-a$ in position $(2n+1-j,2n+1-i)$. The main idea is to conjugate $x$ by a suitable symplectic unipotent matrix to kill off most entries in the first $d$ rows which have a further nonzero entry in the column below them, say in row $i$ for $i>d$.

So suppose that $x$ has at least one nonzero entry in column $j$, with $d \leq j \leq 2n-d$, and suppose further that in this column there is another nonzero entry in position $(i,j)$ for some $i>d$. Then, since $x$ looks the same as $y$ apart from the first $d$ rows and last $d$ columns, one can conclude that:

\begin{enumerate}
	\item[(i)] This other entry is the only other nonzero entry in the $j^{\text{th}}$ column, because $S^d(x)=S^d(y)$ is in standard form.
	\item[(ii)] The position of the entry has relation $d < i < j$ because $x$ is strictly upper triangular.
	\item[(iii)] The entry is a 1 if $i\leq n$ and a $-1$ if $i> n$.
	\item[(iv)] It is the only nonzero entry in the $i^{\text{th}}$ row, except possibly in the last $d$ columns - in particular all entries in row $i$ before the $j^{th}$ column are 0.
\end{enumerate}
To visualise, the $x$ and $y$ are of the following form:
$$\left(\begin{array}{ccc|c|ccc|ccc|ccc|c|ccc}
	&  &  &  & \star & \star & \star & \star & \star & \star & \star & \star & \star &  &  &  &  \\ 
	& J_d &  &  & \star & \star & \star & \star & \star & \star & \star & \star & \star &  &  &  &  \\ 
	&  &  &  & \star & \star & \star & \star & \star & \star & \star & \star & \star &  &  &  &  \\ 
	\hline
	&  &  & \ddots &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  &  &  & \star & \star & \star \\ 
	&  &  &  &  & J_{r-1} &  &  &  &  &  &  &  &  & \star & \star & \star \\ 
	&  &  &  &  &  &  &  &  &  & 1_{(a)} &  &  &  & \star & \star & \star \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  &  &  & \star & \star & \star \\ 
	&  &  &  &  &  &  &  & \tilde{J}_{2s+2} &  &  &  &  &  & \star & \star & \star \\ 
	&  &  &  &  &  &  &  &  &  &  &  &  &  & \star & \star & \star \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  &  &  & \star & \star & \star \\ 
	&  &  &  &  &  &  &  &  &  &  & \!\!\!\!\!\!\!\!-J_{r-1} &  &  & \star & \star & \star \\ 
	&  &  &  &  &  &  &  &  &  &  &  &  &  & \star & \star & \star \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  &  & \ddots &  &  &  \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
	&  &  &  &  &  &  &  &  &  &  &  &  &  &  & -J_d &  \\ 
	&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 
\end{array}\right).$$
Here the entry $1_{(a)}$ is the entry in the bottom-left location of its respective block, and the stars indicate arbitrary entries at any location in their blocks for $x$, but for $y$ the stars indicate only zero-entries at any location in their blocks. In this situation, let $v$ denote the first $d$ rows in the $j^{\text{th}}$ column, viewed as a column vector of length $d$. Let $v_s$ denote every position $s$ of vector $v$. We now split into the following subcases to cover all possibilities:

%As $x'$ is symplectic, any entry $v_t$ in the position $(i,j)$ is matched by $-v_t$ in position $(2n+1-j,2n+1-i)$, so we limit the required work to what partition $x'$ is in whenever there are nonzero entries in the first $d$ rows, for columns $j$ with $j>d$. Now  As established for the details of $\mathfrak{gl}_n$ in section \ref{Sec:GLnAnyMatSize}, let $v$ be the first $d$ rows of the $j^{\text{th}}$ column, and let $v_t=v_{t,j}$ be the last nonzero entry of $v$.
% As $x'$ is in standard form, there is one more nonzero entry in the $j^{\text{th}}$ column, in position $(i,j)$, with $i>d$.

\begin{enumerate}
	\item $j\leq n,$ and $i \leq n,$
	\item $j   > n,$ and $i \leq n,$
	\item $j   > n,$ and $i    > n.$
\end{enumerate}
%\emph{\textcolor{red}{Subcase 1:}}
%%\begin{enumerate}
%%	\item [Subcase 1:]
%if $j\leq n,$ and $i\leq n$, then the case is almost identical to determining the orbit of a nilpotent matrix in $\mathfrak{gl}_n$, see Lemma \ref{Lem:OrbitAnyEntryLocation} \textcolor{red}{Find ref} in Section \ref{Sec:GLnAnyMatSize} \textcolor{red}{Find ref}. Let $v_t$ be the last nonzero entry in the $j^{\text{th}}-{\text{column}}$, more precisely in position $(t,j)$, and the symplectic property requires that $-v_t$ is in position $(2n+1-j,2n+1-t)$. Let $u$ be a unipotent symplectic matrix with $1$s down the diagonal, $-v_t$ in position $(t,i)$, and (since $u$ is symplectic) $v_t$ in position $(2n+1-i,2n+1-t)$. Recall the action of the unipotent matrix on the basis vectors (Equation \ref{eqn:UnipConj} \textcolor{red}{Find ref}):
%
%\begin{align*}
%	u(e_p)&=
%	\begin{cases}
%		e_p-v_te_t	&\text{ if } p=i,\\
%		e_p			&\text{ otherwise.}
%	\end{cases}\\
%	u^{-1}(e_p)&=
%	\begin{cases}
%		e_p+v_te_t	&\text{ if } p=i,\\
%		e_p			&\text{ otherwise.}
%	\end{cases}
%\end{align*}
%Then $$uxu^{-1}(e_i)=ux(e_i+v_te_t)=ux(e_i)+u(v_te_{t-1}),$$
%so a $v_t$-value is added to the entry in position $(t-1,i)$, but no other entries before the $j^{\text{th}}$ column are altered. And 
%$$uxu(e_j)=ux(e_j+\sum_{l=1}^t v_l e_l)=u(e_i-v_te_t+\sum_{l=1}^t v_l e_l)=e_i+\sum_{l=1}^{t-1} v_l e_l.$$
%So the $v_t$-entry in position $(t,j)$ is killed off. Hence by conjugation with $u$, the $v_t$-value in position $(t,j)$ moves up and to the left. 
%
%\emph{\textcolor{red}{Subcase 2:}}	
%%	\item [Subcase 2:]
%if $j >n,$ and $i\leq n$ then the other nonzero entry in the $j^{\text{th}}$ column is found on the anti-diagonal. As before, we will determine a unipotent matrix to conjugate $x$ with, but we calculate what entries can be found in $uxu^{-1}$ for each column, with an example for further clarity. Recall that the second half of the symplectic basis is indexed backwards, $f_1$ is the last basis vector, $f_2$ the second to last, etc, with $f_n$ being the $n+1^{\text{th}}$ basis vector, $f_{n-1}$ being the $n+2^{th}$, etc. As an example, let $n=7, j=9, i=6, t=3$, so: \textcolor{red}{See if the example can be removed}
%
%$$x= \left(
%\begin{array}{cccc|cccccc|cccc}
%	0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%	0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%	0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & v_3 & 0 & 0 & 0 & 0 & 0 \\
%	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%	\hline
%	0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & v_3 & 0 & 0 \\
%	0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\
%	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 & 0 & 0 \\
%	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%	\hline
%	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 & 0 \\
%	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 & 0 \\
%	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -1 \\
%	0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
%\end{array}
%\right).$$
%Note that $x(f_i)=-e_i-v_te_t$, and $x(f_t)=-f_{t+1}-v_te_i$. In this example, $x(f_6)=-e_6-v_te_3$, and $x(f_3)=f_4-v_3e_6$.
%
%Let $u$ be the unipotent matrix with $-v_t$ in position $(t,i)$ and $v_t$ in position $(2n+1-i,2n+1-t)$, then by Equation \ref{eqn:UnipConj} \textcolor{red}{Find reference}, we know that the first $n$ columns of $uxu^{-1}$ are the same as those in $x$, with a $v_t$ removed from position $(t,j)$ and added in position $(t-1,i)$. The calculation of interest is: $uxu^{-1}(e_i)=e_{i-1}+v_te_{t-1}$. By the symplectic property, we also get that the $v_t$ entry in position $(2n+1-j,2n+1-t)$ is removed, and a $-v_t$-value in position $(2n+1-i,2n+2-t)$ is added. To check this, we calculate the conjugation $u\cdot x$ for the last $n$ columns:
%
%\begin{align*}
%	u(f_p)&=
%	\begin{cases}
%		f_p+v_tf_i	&\text{ if } p=t,\\
%		f_p			&\text{ otherwise.}
%	\end{cases}\\
%	u^{-1}(f_p)&=
%	\begin{cases}
%		f_p-v_te_i	&\text{ if } p=t,\\
%		f_p			&\text{ otherwise.}
%	\end{cases}
%\end{align*}
%Checking for the columns $p$ with $n<p<j$, we note that this corresponds to the basis vectors $f_{2n+1-n},f_{2n+1-(n-1)},\ldots,f_{2n+1-(j-1)}$. As $n<j<2n-d$, we get $f_{2n+1-n}>f_{2n+1-p}>f_{2n+1-j}$ and with $t\leq d$, we get $f_{2n+1-j}>f_t$, so $f_{2n+1-p}\neq f_t$ for $n<p<j$. For these $f_{2n+1-p}$ it must follow that $uxu^{-1}(f_{2n+1-p}) = ux(f_{2n+1-p})$. Furthermore, as $x$ is upper triangular, $x(f_{2n-1+p})$ does not involve $f_t$, so $ux(f_{2n+1-p})=x(f_{2n+1-p})$. Next, for $p=j$, we repeat the calculation:
%
%$$uxu^{-1}(f_{2n+1-j})=ux(f_{2n+1-j})=u(-e_i+\sum_{s=1}^t v_se_s)=-e_i-v_te_t+\sum_{s=1}^t v_se_s=-e_i+\sum_{s=1}^{t-1}v_se_s.$$
%In the example, $$uxu^{-1}(f_6)=ux(f_6)=u(-e_6+\sum_{s=1}^3 v_se_s)=-e_6-v_3e_3+\sum_{s=1}^3 v_se_s=-e_i+\sum_{s=1}^2 v_se_s=-e_6.$$
%
%For $p>j, p\neq t-1$ and $p\neq t-1$, we again get $uxu^{-1}(f_p)=x(f_p)$. For $p=t-1$, we have that $uxu^{-1}(f_{t-1})=-f_t-v_tf_i$, hence $uxu^{-1}$ has a $-v_t$-entry in position $(2n+1-i,2n+2-t)$, as $u$ is symplectic. Finally, if $p=t$, we get that $uxu^{-1}(f_t) = ux(f_t-v_tf_i) = u(-f_{t+1}+v_t^2e_t) = -f_{t+1}+v_t^2e_t$, so the $v_t$-entry in position $(2n+1-j,2n+1-t)$ is removed (the $v_t^2$-entry added in $uxu^{1}$, in position $(t, 2n+1-t)$ is not of interest).
%
%To summarize, conjugation by $u$ kills off the $v_t$-entry in position $(t,j)$ at the expense of adding a $v_t$-value to the entry in position $(t-1,i)$, possibly making it nonzero. The other entries of $uxu^{-1}$ before column $j$ are unchanged, hence the $v_t$-value in position $(t,j)$ is moved up and to the left. In particular for Subcase 2, because $t-1 \leq d < n$, and $i \leq n$, the entry where a $v_t$-value is added, is in position $(t-1,i)$. If the entry in this position needs to be removed, subcase 1 can be applied to do so.
%
%\emph{\textcolor{red}{Subcase 3:}}
%%	\item [Subcase 3:]
%in the last subcase, $i,j>n$. As before, the first $d$ rows of column $j$ form vector $v$, with $v_t$ its last nonzero entry in position $(t,j)$. The only nonzero entry in column $j$, after $v$, is $-1$ in position $(i,j)$. With $v_t$ in position $(t,j)$, there is an entry $v_t$ in position $(2n+1-j,2n+1-t)$. Let $u$ be the unipotent matrix with ones on the diagonal, and a $v_t$ entry in positions $(t,i)$ and $(2n+1-i,2n+1-t)$.
%
%Then for any $e_p$, we get  $u(e_p)=e_p$ and $u^{-1}(e_p)=e_p$, so $u$ and $u^{-1}$ do nothing to the first half of the basis, hence the first $n$ columns of $x$ and $uxu^{-1}$ are the same. Next, with $n+1\leq i<j\leq 2n-d$, we let $p$ range as follows ($n+1 \leq p \leq 2n$): 
%
%$$\{n+1,\ldots, i-1,i,i+1,\ldots,2n+1-t,2n-t,\ldots,2n\}.$$
%Then we get the following sequence of basis vectors $f_{2n+1-p}$:
%
%$$\{f_n, \ldots, f_{2n+1-(i-1)}, f_{2n+1-i}, f_{2n+1-(i+1)}, \ldots, f_{t+1}, f_t, f_{t-1},\ldots f_1\},$$
%and the action of $u$ yields:
%
%\begin{align*}
%	u(f_{2n+1-p})&=
%	\begin{cases}
%		f_{2n+1-p}-v_te_t			&\text{ if } p=i,\\
%		f_{2n+1-p}-v_te_{2n+1-i}	&\text{ if } p=2n+1-t,\\
%		f_{2n+1-p}					&\text{ otherwise.}
%	\end{cases}\\
%	u^{-1}(f_{2n+1-p})&=
%	\begin{cases}
%		f_{2n+1-p}+v_te_t			&\text{ if } p=i,\\
%		f_{2n+1-p}+v_te_{2n+1-i}	&\text{ if } p=2n+1-t,\\
%		f_{2n+1-p}					&\text{ otherwise.}
%	\end{cases}	
%\end{align*}
%The sequence of $u(f_{2n+1-p})$ is as follows:
%
%$$\{f_n, \ldots, f_{2n+1-(i-1)}, f_{2n+1-i}-v_te_t, f_{2n+1-(i+1)}, \ldots, f_{t+1}, f_t-v_te_{2n+1-i}, f_{t-1},\ldots f_1\},$$	
%by our assumptions, we have that $t \leq d$ and $j \leq 2n-d$. So when we look at what happens with the vectors $f_{2n+1-p}$ for $n+1 \leq p < j$, with $p \neq i$, this never includes vector $f_t$.
%
%First, for $n+1 \leq p < j$, and $p \neq i$, we get $uxu^{-1}(f_{2n+1-p})=ux(f_{2n+1-p})$. The only nonzero entries in row $i$ occur in column $j$ (as $S^d(x)$ is in standard form) or later (the last $d$ columns). So applying $x$ to $f_{2n+1-p}$ does not yield basis vector $f_{2n+1-i}$, and since $x$ is strictly upper triangular, applying $x$ to $f_{2n+1-p}$ does not yield $f_t$. So $ux(f_{2n+1-p})=x(f_{2n+1-p})$ when $n+1 \leq p < j$, and $p \neq i$. Hence for $n+1 \leq p < j$, and $p \neq i$, we have that the $p^{\text{th}}$ column of $uxu^{-1}$ is the same as the $p^{\text{th}}$ column of $x$.
%
%Second, if $p=i$, then $uxu^{-1}(f_{2n+1-i})=ux(f_{2n+1-i}+v_te_t)=ux(f_{2n+1-i})+ux(v_te_t)$. Since $x$ is upper triangular, $x(f_{2n+1-i})$ yields basis vectors $f_p$, with $p> 2n+1-i$ and vectors $e_p$ with $1 \leq p \leq n$, which are all fixed under $u$. Furthermore $ux(v_te_t)=u(v_te_{t-1})=v_te_{t-1}$, since we know the action of $x$ on $v_te_t$ explicitly, and all $e_p$ vectors are fixed under $u$ ($1 \leq p \leq n$).
%
%So the $i^{\text{th}}$ column of $uxu^{-1}$ is the same as the $i^{\text{th}}$ column of $x$, except a $v_t$-value is added to the entry in position $(t-1,i)$.
%
%Next, let $p=j$, then:
%
%\begin{align*}
%	uxu^{-1}(f_{2n+1-j})	&= u(f_{2n+1-i}+\sum_{s=1}^t v_se_s)\\
%	&= f_{2n+1-i}-v_te_t+\sum_{s=1}^tv_se_s\\
%	&= f_{2n+1-i}+\sum_{s=1}^{t-1}v_se_s.
%\end{align*}
%So conjugating with $u$ removes the $v_t$ value in position $(t,j)$.
%
%Considering the action on the $i^{\text{th}}$ column and the $j^{\text{th}}$ column, conjugation by $u$ kills off the $v_t$-entry in position $(t,j)$, at the expense of adding a $v_t$-value to the entry in position $(t-1,i)$, which may make it nonzero. Except for the change of this value in position $(t-1,i)$, no other entry before column $j$ is altered by the conjugation.
%With these subcases in hand, we can remove nonzero entries $v_t$ in position $(t,j)$ in columns where a further nonzero entry in row $i$ is present. Specifically, by conjugating, the $v_t$-value of the entry in position $(t,j)$ moves up and to the left. By systematically iterating these conjugations, we can kill off all the $v_t$-entries in the first $d$ rows (starting with the entry in position $(d,2n+1-d)$; the last row of the rightmost column), in the columns where a further nonzero entry is present, until the only nonzero entries left in the first $d$ rows are in the columns which have zero entries everywhere else. Since each of the conjugating elements is sent to the identity in the limit, we have that the limit along the ``new'' $x$ is still equal to $y$.
%So we may assume that $x$ is of the following form:
%
%$$x=\left(\begin{array}{ccc|c|ccc|ccc|ccc|c|ccc}
%	&  &  &  & \star &  &  & \star &  &  &  &  &  &  &  &  &  \\ 
%	& J_d &  &  & \star &  &  & \star &  &  &  &  &  &  &  &  &  \\ 
%	&  &  &  & \star &  &  & \star &  &  &  &  &  &  &  &  &  \\ 
%	\hline
%	&  &  & \ddots &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%	\hline
%	&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%	&  &  &  &  & J_{r-1} &  &  &  &  &  &  &  &  &  &  &  \\ 
%	&  &  &  &  &  &  &  &  &  & 1_{(a)} &  &  &  &  &  &  \\ 
%	\hline
%	&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%	&  &  &  &  &  &  &  & \tilde{J}_{2s+2} &  &  &  &  &  &  &  &  \\ 
%	&  &  &  &  &  &  &  &  &  &  &  &  &  & \star & \star & \star \\ 
%	\hline
%	&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%	&  &  &  &  &  &  &  &  &  &  & \!\!\!\!\!\!\!\!-J_{r-1} &  &  &  &  &  \\ 
%	&  &  &  &  &  &  &  &  &  &  &  &  &  & \star & \star & \star \\ 
%	\hline
%	&  &  &  &  &  &  &  &  &  &  &  &  & \ddots &  &  &  \\ 
%	\hline
%	&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%	&  &  &  &  &  &  &  &  &  &  &  &  &  &  & -J_d &  \\ 
%	&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 
%\end{array} \right),$$
%where $1_{(a)}$ is the entry in the bottom-left of its respective block, and the stars indicate arbitrary entries in the first column or last row of their respective blocks (zero entries are omitted as usual). 
%First, we consider the behaviour and orbit of $x$ in an abstract way, then we analyse in detail what change of orbits occurs. While $y$ induces vector chains of size $2r-2, 2s+2$ and two chains of size $d$, matrix $x$ induces different vector chains. Consider the effect of $x$ on a basis vector $f_i$ for $1 \leq i \leq d$. If $x (f_i) \neq 0$, then $f_i$ is in the vector sequence starting with $f_1$, and the value of $f_i$ is added to a vector from another vector sequence in the center of the matrix. In other words, a vector sequence initiated in the $[d]$ part at the bottom of the matrix will be continued by the $J_{2r-2}$ Jordan blocks or the $J_{2s+2}$ Jordan block in the central portion of the matrix, where in the matrix $y$ the vector chains of parts $[2r-2]$ and $[2s+2]$ are initiated. By the symplectic property, the vector chains of lengths $2r-2$ and $2s+2$ that are terminated in $y$ are picked up by the $J_d$ Jordan block at the top left of the matrix. In detail, the following moves occur, in two cases:
%
%\emph{Case 1:} if $s >d$, then $x$ induces vector chains of size $s+2a$, $r+2b$ and two chains of size $d-a-b$, with at least one of $a$ and $b$ nonzero. So taking $\lim_\lambda x$ is a move of type 2, in fact two moves of type 2 occur simultaneously:
%
%$$\mathcal{O}([r+2a,s+2b,d-a-b,d-a-b])\rightarrow \mathcal{O}([r,s,d,d]),$$	
%is a combination of
%
%\begin{align*}
%	\mathcal{O}([r+2a,s+2b,d-a-b,d-a-b]) &\rightarrow \mathcal{O}([r,s+2b,d-b,d-b]),\\
%	\mathcal{O}([r,s+2b,d-b,d-b]) &\rightarrow \mathcal{O}([r,s,d,d]).
%\end{align*}
%\emph{Case 2:} if $d > r$, then we analyse the matrix $x$ separately for even $d$ and for odd $d$. Without loss of generality, we can assume that the nonzero entry is in the first column after the $[d]$ block, so in the otherwise zero column of the $J_{2r-2}$ block. If $d$ is even, let $d=2d'$, and denote top left $2d' \times (2d'+1)$ block of matrix $x$ as follows:
%
%$$\left(\begin{array}{ccccccccc|c}
%	&  &  &  &  &  &  &  &  & x_{1,2d'+1} \\ 
%	&  &  &  &  &  &  &  &  & \vdots \\ 
%	&  &  &  &  &  &  &  &  & x_{k,2d'+1} \\ 
%	&  &  &  &  &  &  &  &  & x_{k+1,2d'+1} \\ 
%	&  &  &  & J_d &  &  &  &  & \vdots \\ 
%	&  &  &  &  &  &  &  &  & x_{k+i+,2d'+1} \\ 
%	&  &  &  &  &  &  &  &  & x_{k+i+1,2d'+1} \\ 
%	&  &  &  &  &  &  &  &  & \vdots \\ 
%	&  &  &  &  &  &  &  &  & x_{k+i+j,2d'+1}\\
%	\hline\end{array}\right),$$
%here we let $k, i$ and $j$ take their maximum value, and we now relate the orbit of $x$ to the position of the nonzero entry, and determine in what values $k, i$ and $j$ range.
%
%If we consider a single nonzero entry, in a row $k+i+j$, we start by considering the last row; row $d=2d'$ Then $x$ has a Jordan block of size $2d'+2d'+2r-2$ (and a Jordan block of size $2s+2$, which is not involved). Then, if we consider the nonzero entry to be in one row higher, this part loses two pieces to two different parts, so $x$ has parts of size $2d'+2d'+2r-4$, and there are now two parts of size $1$. For every row higher, the largest part loses two additional pieces to the two smaller parts, until these are of size $2r-2$, hence $x$ is in the orbit of $[2d'+2d'-(2r-2),2r-2,2r-2,2s+2]$. Hence, if the nonzero entry is in one of these last $2r-2$ rows, taking the limit $\lim_\lambda x$ yields the move: 
%$$\mathcal{O}([2d'+2d'+(2r-2)-2j,j,j,2s+2]) \rightarrow \mathcal{O}([2d',2d',2r-2,2s+2]),$$
%which is a move of type 2. Furthermore, we have determined that $1 \leq j \leq 2r-2$.
%
%Next, if we consider the nonzero entry to be another row higher, the first part loses two pieces and the second part gains two pieces, hence taking $\lim_\lambda x$ gives the following move: $\mathcal{O}([2d'+2d'-(2r-2)-2,2r-2+2,2r-2,2s+2]) \rightarrow \mathcal{O}([2d',2d',2r-2,2s+2])$. Then, for every row we go up, the first part will be two additional pieces smaller, and the second part will be two additional pieces bigger, hence if the nonzero entry is in row $2d'-(2r-2)-i$, $x$ is in the orbit of $[2d'+2d'-(2r-2)-2i,2r-2+2i,2r-2,2s+2]$, and taking the limit $\lim_\lambda x$ yields the move:
%$$\mathcal{O}([2d'+2d'-(2r-2)-2i,2r-2+2i,2r-2,2s+2])\rightarrow \mathcal{O}([2d',2d',2r-2,2s+2]),$$
%which is a move of type 1. This is possible until $2i=2d'-(2r-2)$, because when this equality holds, $x$ is in the orbit of $[2d',2d',2r-2,2s+2]$, which is the same orbit as $y=\lim_\lambda x$, and no move occurs. Hence we have determined that $1 \leq i \leq d'-(r-1)$, and then for the maximum values of $i$ and $j$, we determine that the range of $k$ is as follows: $1\leq k \leq 2d'-i-j = d'-(r-1)$. We can now make the following conclusion:
%
%\begin{enumerate}
%	\item[(i)] If the nonzero entry is in position $k$, for $1\leq k \leq 2d'-i-j = d'-(r-1)$, then $x$ is in the orbit of $[2d',2d',2r-2,2s+2]$. Taking $\lim_\lambda x$ will not change the orbit.
%	\item[(ii)] If the nonzero entry is in position $k+i$ for the maximum value of $k$ and $1 \leq i \leq d - (r-1)$, then $x$ is in the orbit of $[2d'+2i,2d'-2i,2r-2,2s+2]$. Taking $\lim_\lambda x$ is a move of type $1$, where the $[2r-2]$ and $[2s+2]$ pieces are unchanged.
%	\item[(iii)] If the nonzero entry is in position $k+i+j$ for maximum values of $k,i$, and $1 \leq j \leq 2r-2$, then $x$ is in the orbit of $[2d'+2i+2j,2d'-di-j,2r-2-j]$. Taking $\lim_\lambda x$ is a combination of move $1$ and move $2$: $\mathcal{O}([2d'+2i+2j,2d'-di-j,2r-2-j]) \rightarrow \mathcal{O}([2d'+2i,2d'-di,2r-2]) \rightarrow \mathcal{O}([2d,2d,2r-2,2s+2])$.
%\end{enumerate}
%
%If $d$ is odd, we denote $d=2d'+1$, and this introduces a row where the nonzero entry places $x$ in the orbit of $[2d'+1,2d'-1,r-2,s+2].$ Then the conclusion changes only by the size of the blocks:
%
%\begin{enumerate}
%	\item[(i)] If the nonzero entry is in position $k$, for $k \leq d' -(r-1)$, then $x$ is in the orbit of $[2d'+1,2d'+1,2r-2,2s+2]$. Taking $\lim_\lambda x$ will not change the orbit.
%	\item[(ii)] If the nonzero entry is in position $k+i$ for the maximum value of $k$ and $1 \leq i \leq d - (r-1)+1$, then $x$ is in the orbit of $[2d'+1+(2(i-1)+1),2d'-(2(i-1)-1),2r-2,2s+2]$. Taking $\lim_\lambda x$ is a move of type $1$, where the $[2r-2]$ and $[2s+2]$ blocks are unchanged.
%	\item[(iii)] If the nonzero entry is in position $k+i+j$ for maximum values of $k,i$, and $1 \leq j \leq 2r-2$, then $x$ is in the orbit of $[2d'+(2(i-1)+1)+2j,2d'-(2(i-1)+1)-j,2r-2-j]$. Taking $\lim_\lambda x$ is a combination of move $1$ and move $2$: $\mathcal{O}([2d'+(2(i-1)+1)+2j,2d'-(2(i-1)+1)-j,2r-2-j]) \rightarrow \mathcal{O}([2d'+2i,2d'-di,2r-2]) \rightarrow \mathcal{O}([2d,2d,2r-2,2s+2])$.
%\end{enumerate}
%We now have determined the move for a nonzero entrey in the $d+1^{\text{th}}$ column: a nonzero entry in the first $d$ rows of the first column above the $J_{r-1}$ Jordan block gives rise to a move involving the parts that are of size $[d]$ and $[2r-2]$ after taking the limit, and we have also established that it does not involve the part of size $[2s+2]$. Similarly, a nonzero entry in the first column above the $\tilde{J}_{2s+2}$ Jordan block gives rise to a move involving the parts that are of size $[d]$ and $[2s+2]$ after taking the limit, but it doesn't involve the part of size $[2r-2]$.
%
%In the case there are nonzero entries in the first columns above both Jordan blocks, taking the limit will give rise to two moves, that separately involve the parts which (after taking the limit) are of size $[2s+2]$ and $[d]$, and the parts which are of size $[2r-2]$ and $[d]$. However, the nonzero entries do not allow for a move between the parts that are of size $[2r-2]$ and $[2s+2]$, after taking the limit. Hence in this special case, the required move does not occur.
%
%So for both case 1 and case 2, the nonzero entries described are only in the first $d$ rows of the matrix so the move only involves the $[2r-2]$ and $[d]$ parts when the nonzero entries are above the $J_{r-1}$ bock. In case the nonzero entries are above the $J_{2s+2}$ block, the move involves the $[2s+2]$ and $[d]$ blocks.
%
%We will now generalize as we go down the diagonal, where the $J_{d_i}$ blocks are present, for $1 \leq i \leq m$. The nonzero entries in the first column above the $J_{r-1}$ blocks are next to the $J_{d_i}$ blocks, so we obtain a move involving the $[2r-2]$ and $[d_i]$ parts (after taking the limit). Regardless of the details of the move, the $[2s+2]$ part is not involved.
%
%Vice versa, the nonzero entries in the first column above the $J_{2s+2}$ Jordan block, in any row of one of the $J_d$ or $J_{d_i}$ Jordan blocks give rise to a move involving the parts $[2s+2],[d],[d_1],\ldots,[d_m]$ (after taking the limit), but the $[2r-2]$ part is not involved.
%
%Hence, regardless of the location of the nonzero entries above the $J_{r-1}$ and $\tilde{J}_{2s+2}$ Jordan block, a move of type $[2r,2s]\rightarrow [2r-2,s2+2]$ does not occur.
%
%This shows that the move $\mathcal{O}([\ldots,r,s,\ldots])\rightarrow \mathcal{O}([\ldots,r-2,s+2,\ldots])$ does not occur. We conclude that the orbit $\mathcal{O}([\ldots,r-2,s+2,\ldots])$ is not accessible from the orbit $\mathcal{O}([\ldots,r,s,\ldots])$.
%\end{proof}
\emph{Subcase 1:} if $j\leq n,$ and $i\leq n$, then the case is almost identical to determining the orbit of a nilpotent matrix in $\mathfrak{gl}_n$, see Lemma \ref{Lem:OrbitAnyEntryLocation} \textcolor{red}{Find ref} in Section \ref{Sec:GLnAnyMatSize} \textcolor{red}{Find ref}. Let $v_t$ be the last nonzero entry in the $j^{\text{th}}-{\text{column}}$, more precisely in position $(t,j)$, and the symplectic property requires that $-v_t$ is in position $(2n+1-j,2n+1-t)$. Let $u$ be a unipotent symplectic matrix with $1$s down the diagonal, $-v_t$ in position $(t,i)$, and (since $u$ is symplectic) $v_t$ in position $(2n+1-i,2n+1-t)$. The action of the unipotent matrix on the basis vectors is as follows:

\begin{align}\label{eqn:UnipConj}
	u(e_p)&=
	\begin{cases}
		e_p-v_te_t	&\text{ if } p=i,\\
		e_p			&\text{ otherwise.}
	\end{cases}\\
	u^{-1}(e_p)&=
	\begin{cases}
		e_p+v_te_t	&\text{ if } p=i,\\
		e_p			&\text{ otherwise.}
	\end{cases}
\end{align}
Then byu calculating $uxu^{-1}(e_p)$ for $0 \leq p \leq n$, it becomes clear that conjugation removes the $v_t$ entry in position $(t-1,j-1)$, and adds a $v_t$-value to the entry in position $(t-1,j-1)$, hence the $v_t$-entry moves one place up and to the left. As $x$ and $u$ are symplectic, the $-v_t$-value in position $(2n+1-j,2n+1-t)$ moves one place down and to the right.

\emph{subcase 2:} if $j >n,$ and $i\leq n$ then the other nonzero entry in the $j^{\text{th}}$ column is found on the anti-diagonal. As before, we will determine a unipotent matrix to conjugate $x$ with, but we calculate what entries can be found in $uxu^{-1}$ for each column, with an example for further clarity. Recall that the second half of the symplectic basis is indexed backwards, $f_1$ is the last basis vector, $f_2$ the second to last, etc, with $f_n$ being the $n+1^{\text{th}}$ basis vector, $f_{n-1}$ being the $n+2^{th}$, etc.

Note that $x(f_i)=-e_i-v_te_t$ and $x(f_t)=-f_{t+1}-v_te_i$. Let $u$ be the unipotent matrix with $-v_t$ in position $(t,i)$ and $v_t$ in position $(2n+1-i,2n+1-t)$, then by Equation, the action of $u$ on vectors $e_p$ is known, hence the first $n$ columns of $uxu^{-1}$ are almost the same as those in $x$; with a $v_t$-value added to the entry in position $(t-1,i)$. The calculation of interest is: $uxu^{-1}(e_i)=e_{i-1}+v_te_{t-1}$. To check that the $v_t$-entry is removed from position $(t,j)$, the conjugation $uxu^{-1}(f_{2n+1-j})$ needs to be checked (note that $2n+1-j=i$). The action of $u$ on the vectors $f_p$ is:

\begin{align*}
	u(f_p)&=
	\begin{cases}
		f_p+v_tf_i	&\text{ if } p=t,\\
		f_p			&\text{ otherwise.}
	\end{cases}\\
	u^{-1}(f_p)&=
	\begin{cases}
		f_p-v_te_i	&\text{ if } p=t,\\
		f_p			&\text{ otherwise.}
	\end{cases}
\end{align*}
So $u(f_{2n+1-j})=u(f_i)=f_i$, and the calculation of interest is: $uxu^{-1}(f_i)=-f_{i+1}+\sum_{s=1}^{t-1}v_se_s$ (the last nonzero element of the column designated as $v$ has been changed to zero). Hence conjugation with $u$ removes the $v_t$-entry from position $(t,j)$. So here, the $v_t$ value also moves up and to the left in the matrix. In particular for Subcase 2, because $t-1 \leq d < n$, and $i \leq n$, the entry where a $v_t$-value is added, is in position $(t-1,i)$. If the entry in this position needs to be removed, subcase 1 can be applied to do so. Note that $x$ and $u$ are symplectic, so there is also a $v_t$ entry in position $(2n+1-j,2n+1-t)$ that is moved to position $(2n+1-i,2n+2-t)$.
\textcolor{red}{Mention there is a $v_t^2$ added somewhere but that this is not important}

\emph{subcase 3:} if $i,j>n$, then the other nonzero entry in the $j^\text{th}$ column has value $-1$. As usual, let $v$ be the vector of the first $d$ entries of the $j^\text{th}$ column. With $v_t$ in position $(t,j)$, there is an entry $v_t$ in position $(2n+1-j,2n+1-t)$. Let $u$ be the unipotent matrix with ones on the diagonal, and a $v_t$ entry in positions $(t,i)$ and $(2n+1-i,2n+1-t)$. Second, note that $u(e_p)=u^{-1}(e_p)=e_p$ for all $p$, so the first $n$ columns of $x$ and $uxu^{-1}$ are the same. Next, let $p$ range from $n+1$ to $2n$, and denote the second half of the basis as follows:
$$\{f_n, \ldots, f_{2n+1-(i-1)}, f_{2n+1-i}, f_{2n+1-(i+1)}, \ldots, f_{t+1}, f_t, f_{t-1},\ldots f_1\},$$
then the action of $u$ yields:
\begin{align*}
	u(f_{2n+1-p})&=
	\begin{cases}
		f_{2n+1-p}-v_te_t			&\text{ if } p=i,\\
		f_{2n+1-p}-v_te_{2n+1-i}	&\text{ if } p=2n+1-t,\\
		f_{2n+1-p}					&\text{ otherwise.}
	\end{cases}\\
	u^{-1}(f_{2n+1-p})&=
	\begin{cases}
		f_{2n+1-p}+v_te_t			&\text{ if } p=i,\\
		f_{2n+1-p}+v_te_{2n+1-i}	&\text{ if } p=2n+1-t,\\
		f_{2n+1-p}					&\text{ otherwise.}
	\end{cases}	
\end{align*}
So the calculations of interest are $u(f_{2n+1-i})=f_{2n+1-i}-v_te_t$, and $u(f_t)=f_t-v_te_{2n+1-i}$. As $t \leq d$ and $j \leq 2n-d$, vectors $f_{2n+1-p}$, for $n+1\leq p< j$ and $p\neq i$, never include $f_t$, hence for these values of $p$, one gets $uxu^{-1}(f_{2n+1-p})=ux(f_{2n+1-p})$. Furthermore for these values of $p$, $x(f_{2n+1-p})$ never yields $f_{2n+1-i}$ (the only nonzero in row $i$ occurs in column $j$ or later), and never yields $f_t$ (since $x$ is strictly upper triangular). Hence $x(f_{2n+1-p})$ is invariant under $u$ for $n+1\leq p< j$ and $p\neq i$, so $ux(f_{2n+1-p})=x(f_{2n+1-p})$. Third, if $p=i$, then $uxu^{-1}(f_{2n+1-i})=ux(f_{2n+1-i}+v_te_t)=ux(f_{2n+1-i})+ux(v_te_t)$. Since $x$ is upper triangular, $x(f_{2n+1-i})$ yields $f_p$ (with $p> 2n+1-i)$ and $e_p$ ($p\leq n$), both fixed under $u$. Furthermore, $ux(v_te_t)=u(v_te_{t-1})=v_te_{t-1}$, since the action of $x$ on $v_te_t$ is known explicitly, and all $e_p$ are fixed under $u$. Hence conjugation with $u$ adds a $v_t$ value to the $(t-1,i)$ entry. Finally, if $p=j$ then:
\begin{align*}
	uxu^{-1}(f_{2n+1-j})	&= u(f_{2n+1-i}+\sum_{s=1}^t v_se_s)\\
	&= f_{2n+1-i}-v_te_t+\sum_{s=1}^tv_se_s\\
	&= f_{2n+1-i}+\sum_{s=1}^{t-1}v_se_s.
\end{align*}
So conjugation again removes the $v_t$ entry from position $(t,j)$. The conclusion is that in subcase 3, the conjugation also removes the $v_t$ entry in position $(t,j)$ and adds a $v_t$ value to the entry in position $(t-1,i)$. Since $x$ and $u$ are symplectic, the $v_t$ entry in position $(2n+1-j,2n+1-t)$ is also removed, and a $v_t$ value is added to position $(2n+1-i,2n+2-t)$.

All three subcases together allow for repeated conjugation to remove nonzero entries from positions $(t,j)$ with $t \leq d$, and $d+1\leq j \leq 2n-d$, if a further nonzero element is present in column $j$, specifically in position $(i,j)$ with $i>d$. This is at the expense of adding a $v_t$ value to the entry in position $(t-1,i)$, which can be understood as moving the $v_t$ values up and to the left in the matrix. This process is repeated until there only nonzero entries in the first $d$ rows, in columns that have no nonzero entry further down (after row $d$). So the matrix can be conjugated until it is of the form:
$$x=\left(\begin{array}{ccc|c|ccc|ccc|ccc|c|ccc}
	&  &  &  & \star &  &  & \star &  &  &  &  &  &  &  &  &  \\ 
	& J_d &  &  & \star &  &  & \star &  &  &  &  &  &  &  &  &  \\ 
	&  &  &  & \star &  &  & \star &  &  &  &  &  &  &  &  &  \\ 
	\hline
	&  &  & \ddots &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
	&  &  &  &  & J_{r-1} &  &  &  &  &  &  &  &  &  &  &  \\ 
	&  &  &  &  &  &  &  &  &  & 1_{(a)} &  &  &  &  &  &  \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
	&  &  &  &  &  &  &  & \tilde{J}_{2s+2} &  &  &  &  &  &  &  &  \\ 
	&  &  &  &  &  &  &  &  &  &  &  &  &  & \star & \star & \star \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
	&  &  &  &  &  &  &  &  &  &  & \!\!\!\!\!\!\!\!-J_{r-1} &  &  &  &  &  \\ 
	&  &  &  &  &  &  &  &  &  &  &  &  &  & \star & \star & \star \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  &  & \ddots &  &  &  \\ 
	\hline
	&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
	&  &  &  &  &  &  &  &  &  &  &  &  &  &  & -J_d &  \\ 
	&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 
\end{array} \right),$$
where $1_{(a)}$ is the entry in the bottom-left of its respective block, and the stars indicate arbitrary entries in the first column or last row of their respective blocks (zero entries are omitted as usual). 
First, the behaviour and orbit of $x$ are checked in an abstract way, a detailed analysis of the orbit changes follows afterwards. While $y$ induces vector chains of size $2r-2, 2s+2$ and two chains of size $d$, matrix $x$ induces different vector chains. Consider the effect of $x$ on a basis vector $f_i$ for $1 \leq i \leq d$. If $x (f_i) \neq 0$, then $f_i$ is in the vector sequence starting with $f_1$, and the value of $f_i$ is added to a vector from another vector sequence in the center of the matrix. In other words, a vector sequence initiated in the $J_d$ Jordan block at the bottom of the matrix will be continued by the $J_{2r-2}$ Jordan blocks or the $J_{2s+2}$ Jordan block in the central portion of the matrix, where in the matrix $y$ the vector chains of parts $[2r-2]$ and $[2s+2]$ are initiated. By the symplectic property, the vector chains of lengths $2r-2$ and $2s+2$ that are terminated in $y$ are picked up by the $J_d$ Jordan block at the top left of the matrix. This shows that matrix $x$ has parts $[d-a-b]$ (with multiplicity $2$), $[2r-2+2a]$ and $[2s+2+2b]$ for some $a$ and $b$, contradicting the assumption, hence the move described is not of type 5.

In detail, the following moves occur, in two cases:
\emph{Case 1:} if $s >d$, then $x$ induces vector chains of size $s+2a$, $r+2b$ and two chains of size $d-a-b$, with at least one of $a$ and $b$ nonzero. So taking $\lim_\lambda x$ is a move of type 2, in fact two moves of type 2 occur simultaneously:

$$\mathcal{O}([r+2a,s+2b,d-a-b,d-a-b])\rightarrow \mathcal{O}([r,s,d,d]),$$	
is a combination of

\begin{align*}
	\mathcal{O}([r+2a,s+2b,d-a-b,d-a-b]) &\rightarrow \mathcal{O}([r,s+2b,d-b,d-b]),\\
	\mathcal{O}([r,s+2b,d-b,d-b]) &\rightarrow \mathcal{O}([r,s,d,d]).
\end{align*}
\emph{Case 2:} if $d > r$, then there are two subcases, for even $d$ and odd $d$. Without loss of generality, one can assume that the nonzero entry is in the first column after the $[d]$ block, so in the otherwise zero column of the $J_{2r-2}$ block. If $d$ is even, let $d=2d'$, and denote top left $2d' \times (2d'+1)$ block of matrix $x$ as follows:

$$\left(\begin{array}{ccccccccc|c}
	&  &  &  &  &  &  &  &  & x_{1,2d'+1} \\ 
	&  &  &  &  &  &  &  &  & \vdots \\ 
	&  &  &  &  &  &  &  &  & x_{k,2d'+1} \\ 
	&  &  &  &  &  &  &  &  & x_{k+1,2d'+1} \\ 
	&  &  &  & J_d &  &  &  &  & \vdots \\ 
	&  &  &  &  &  &  &  &  & x_{k+i+,2d'+1} \\ 
	&  &  &  &  &  &  &  &  & x_{k+i+1,2d'+1} \\ 
	&  &  &  &  &  &  &  &  & \vdots \\ 
	&  &  &  &  &  &  &  &  & x_{k+i+j,2d'+1}\\
	\hline\end{array}\right),$$
let $k, i$ and $j$ take their maximum value, relate the orbit of $x$ to the position of the nonzero entry, and determine in what values $k, i$ and $j$ range.

When considering a single nonzero entry, in a row $k+i+j$, first check the last row; row $d=2d'$. Then $x$ has a Jordan block of size $2d'+2d'+2r-2$ (and a Jordan block of size $2s+2$, which is not involved). Then, if one considers the nonzero entry to be in one row higher, this part loses two pieces to two different parts, so $x$ has parts of size $2d'+2d'+2r-4$, and there are now two parts of size $1$. For every row higher, the largest part loses two additional pieces to the two smaller parts, until these are of size $2r-2$, hence $x$ is in the orbit of $[2d'+2d'-(2r-2),2r-2,2r-2,2s+2]$. So, if the nonzero entry is in one of these last $2r-2$ rows, taking the limit $\lim_\lambda x$ yields the move: 
$$\mathcal{O}([2d'+2d'+(2r-2)-2j,j,j,2s+2]) \rightarrow \mathcal{O}([2d',2d',2r-2,2s+2]),$$
which is a move of type 2. Furthermore, we have determined that $1 \leq j \leq 2r-2$.

Next, if the nonzero entry is another row higher, the first part loses two pieces and the second part gains two pieces, hence taking $\lim_\lambda x$ gives the following move: $\mathcal{O}([2d'+2d'-(2r-2)-2,2r-2+2,2r-2,2s+2]) \rightarrow \mathcal{O}([2d',2d',2r-2,2s+2])$. Then, for every the nonzero entry goes up, the first part will be two additional pieces smaller, and the second part will be two additional pieces bigger, hence if the nonzero entry is in row $2d'-(2r-2)-i$, $x$ is in the orbit of $[2d'+2d'-(2r-2)-2i,2r-2+2i,2r-2,2s+2]$, and taking the limit $\lim_\lambda x$ yields the move:
$$\mathcal{O}([2d'+2d'-(2r-2)-2i,2r-2+2i,2r-2,2s+2])\rightarrow \mathcal{O}([2d',2d',2r-2,2s+2]),$$
which is a move of type 1. This is possible until $2i=2d'-(2r-2)$, because when this equality holds, $x$ is in the orbit of $[2d',2d',2r-2,2s+2]$, which is the same orbit as $y=\lim_\lambda x$, and no move occurs. Hence for $1 \leq i \leq d'-(r-1)$, and then for the maximum values of $i$ and $j$, the range of $k$ is as follows: $1\leq k \leq 2d'-i-j = d'-(r-1)$. With this, the following conclusion is reached:

\begin{enumerate}
	\item[(i)] If the nonzero entry is in position $k$, for $1\leq k \leq 2d'-i-j = d'-(r-1)$, then $x$ is in the orbit of $[2d',2d',2r-2,2s+2]$. Taking $\lim_\lambda x$ will not change the orbit.
	\item[(ii)] If the nonzero entry is in position $k+i$ for the maximum value of $k$ and $1 \leq i \leq d - (r-1)$, then $x$ is in the orbit of $[2d'+2i,2d'-2i,2r-2,2s+2]$. Taking $\lim_\lambda x$ is a move of type $1$, where the $[2r-2]$ and $[2s+2]$ pieces are unchanged.
	\item[(iii)] If the nonzero entry is in position $k+i+j$ for maximum values of $k,i$, and $1 \leq j \leq 2r-2$, then $x$ is in the orbit of $[2d'+2i+2j,2d'-di-j,2r-2-j]$. Taking $\lim_\lambda x$ is a combination of move $1$ and move $2$: $\mathcal{O}([2d'+2i+2j,2d'-di-j,2r-2-j]) \rightarrow \mathcal{O}([2d'+2i,2d'-di,2r-2]) \rightarrow \mathcal{O}([2d,2d,2r-2,2s+2])$.
\end{enumerate}

If $d$ is odd, we denote $d=2d'+1$, and this introduces a row where the nonzero entry places $x$ in the orbit of $[2d'+1,2d'-1,r-2,s+2].$ Then the conclusion changes only by the size of the blocks:

\begin{enumerate}
	\item[(i)] If the nonzero entry is in position $k$, for $k \leq d' -(r-1)$, then $x$ is in the orbit of $[2d'+1,2d'+1,2r-2,2s+2]$. Taking $\lim_\lambda x$ will not change the orbit.
	\item[(ii)] If the nonzero entry is in position $k+i$ for the maximum value of $k$ and $1 \leq i \leq d - (r-1)+1$, then $x$ is in the orbit of $[2d'+1+(2(i-1)+1),2d'-(2(i-1)-1),2r-2,2s+2]$. Taking $\lim_\lambda x$ is a move of type $1$, where the $[2r-2]$ and $[2s+2]$ blocks are unchanged.
	\item[(iii)] If the nonzero entry is in position $k+i+j$ for maximum values of $k,i$, and $1 \leq j \leq 2r-2$, then $x$ is in the orbit of $[2d'+(2(i-1)+1)+2j,2d'-(2(i-1)+1)-j,2r-2-j]$. Taking $\lim_\lambda x$ is a combination of move $1$ and move $2$: $\mathcal{O}([2d'+(2(i-1)+1)+2j,2d'-(2(i-1)+1)-j,2r-2-j]) \rightarrow \mathcal{O}([2d'+2i,2d'-di,2r-2]) \rightarrow \mathcal{O}([2d,2d,2r-2,2s+2])$.
\end{enumerate}
Now a conclusion can be drawn regarding the move $\mathcal{O}(x) \rightarrow \mathcal{O}(y)$, given there is a a nonzero entrey in the $d+1^{\text{th}}$ column: a nonzero entry in the first $d$ rows of the first column above the $J_{r-1}$ Jordan block gives rise to a move involving the parts that are of size $[d]$ and $[2r-2]$ after taking the limit, and we have also established that it does not involve the part of size $[2s+2]$. Similarly, a nonzero entry in the first column above the $\tilde{J}_{2s+2}$ Jordan block gives rise to a move involving the parts that are of size $[d]$ and $[2s+2]$ after taking the limit, but it doesn't involve the part of size $[2r-2]$.

In the case there are nonzero entries in the first columns above both Jordan blocks, taking the limit will give rise to two moves, that separately involve the parts which (after taking the limit) are of size $[2s+2]$ and $[d]$, and the parts which are of size $[2r-2]$ and $[d]$. However, the nonzero entries do not allow for a move between the parts that are of size $[2r-2]$ and $[2s+2]$, after taking the limit. Hence in this special case, the required move does not occur.

So for both case 1 and case 2, the nonzero entries described are only in the first $d$ rows of the matrix so the move only involves the $[2r-2]$ and $[d]$ parts when the nonzero entries are above the $J_{r-1}$ bock. In case the nonzero entries are above the $J_{2s+2}$ block, the move involves the $[2s+2]$ and $[d]$ blocks.

In general, there are $J_{d_i}$ blocks present along the diagonal, for $1 \leq i \leq m$. The nonzero entries in the first column above the $J_{r-1}$ blocks are next to the $J_{d_i}$ blocks, so the move involves the $[2r-2]$ and $[d_i]$ parts (after taking the limit). Regardless of the details of the move, the $[2s+2]$ part is not involved.

Vice versa, the nonzero entries in the first column above the $J_{2s+2}$ Jordan block, in any row of one of the $J_d$ or $J_{d_i}$ Jordan blocks give rise to a move involving the parts $[2s+2],[d],[d_1],\ldots,[d_m]$ (after taking the limit), but the $[2r-2]$ part is not involved.

Hence, regardless of the location of the nonzero entries above the $J_{r-1}$ and $\tilde{J}_{2s+2}$ Jordan block, a move of type $[2r,2s]\rightarrow [2r-2,s2+2]$ does not occur.

This shows that the move $\mathcal{O}([\ldots,r,s,\ldots])\rightarrow \mathcal{O}([\ldots,r-2,s+2,\ldots])$ does not occur; the conclusion is that the orbit $\mathcal{O}([\ldots,r-2,s+2,\ldots])$ is not accessible from the orbit $\mathcal{O}([\ldots,r,s,\ldots])$.
\end{proof}

\subsection{Conclusion for $\mathfrak{sp}_{2n}$}
In this section, the five minimal moves in the dominance order of partitions corresponding to symplectic nilpotent orbits have been analysed. These can now describe the order of the orbits in the symplectic algebras. In Section \ref{Sec:GLnConclusion} \textcolor{red}{Find Ref}, the conclusion for accessibility of nilpotent orbits in the general linear group is that the partial order on orbits is the same as the dominance order. This is not the case for the symplectic algebra, as section \ref{Subsec:NonMove} shows that distinguished partitions are not accessible from partitions higher up in the dominance order (e.g. in $\mathfrak{sp}_8$, $\pi_1=[6,2]$ is not accessible from $\pi_2=[8]$). Moreover, if there are two partitions $\pi_1=[\dots,r,s,\ldots]$ and $\pi_2=[\ldots,r-2,s+2,\ldots]$, with $r \geq s+6$, then $\pi_1$ dominates $\pi_2$, but $\pi_2$ is not accessible from $\pi_1$. Since moves 1 -- 4 are valid in the accessibility order (see Section \ref{SympPartitionsMoves}), they give rise to a theorem:

\begin{theorem}\label{Thm:SymplecticAccessibility}
	The partial order on nilpotent symplectic orbits given by the accessibility relation is determined by a combination of the moves of type 1 -- 4.
	%	The accessibility relation gives a partial order on nilpotent orbits in the symplectic groups. The diagram for this partial order comes from joining partitions according to a combination of moves of the types 1 -- 4.
\end{theorem}
 With the proof of Lemma \ref{Lem:AccessibilityPOAlgClosed} (which tells us that the accessibility order is a partial order over algebraically closed $\kappa$), the accessibility order in the symplectic group can now be related to its dominance order:
\begin{lemma}\label{Lem:SPAccOrderDomOrder}
	Let $x,y$ be two nilpotent symplectic matrices. Then $\overline{\mathcal{O}(y)}^c\leq \overline{\mathcal{O}(y)}^c$ if $\overline{\mathcal{O}(y)}\leq \overline{\mathcal{O}(x)}$, unless the move from $\mathcal{O}(x)$ to $\mathcal{O}(x)$ is of type 5.
\end{lemma}
%\begin{proof}
%	We have shown that moves of types 1 -- 4 between adjacent parts of partitions are possible, and the only other type of move cannot occur. It is clear that the order given by $\mathcal{O}(y) \leq \mathcal{O}(x)$ if and only if $\mathcal{O}(y)$ is accessible from $\mathcal{O}(x)$, is reflexive (starting at $x$, and going along the limit of the trivial cocaracter yields $x$ as a result) and transitive (by definition, if $\mathcal{O}(y)$ can be reached from $\mathcal{O}(x)$ using a sequence of cocharacters, and if $\mathcal{O}(z)$ can be reached from $\mathcal{O}(y)$ by a sequence, then $\mathcal{O}(z)$ can be reached from $\mathcal{O}(x)$).
%	
%	The trivial property required for a partial order is antisymmetry, which is clear when we consider $x\in \mathcal{O}(x)$, $y\in \mathcal{O}(y)$ and a cocharacter $\lambda$. If going along the limit of $\lambda$ kills off an entry in $\lambda \cdot x$ to yield $y$, then it brings us strictly down the order of accessibility; no cocharacter $\lambda'$ can reverse the process. Hence if we have $\mathcal{O}(x) \leq \mathcal{O}(y)$ and $\mathcal{O}(y)\leq \mathcal{O}(x)$, it must follow that $\mathcal{O}(x)=\mathcal{O}(y)$.
%\end{proof}
This Theorem answers Questions 1 and 2 in Section \ref{enum:questions}.
\begin{enumerate}
	\item[1] The preorder on orbits given by cocharacter closure is a partial order.
	\item[2] Over a closed field $\overline{\kappa}$, the cocharacter-closure $\overline{G\cdot x}^c$ does not coincide with the Zariski-closure if the Zariski-closure contains a distinguished orbit, or if the Zariski-closure contains an orbit $G\cdot y$, where the move between $\mathcal{O}(x)$ and $\mathcal{O}(y)$ is of type 5.
\end{enumerate}
The difference between the dominance order and the accessibility order of orbits, can be described as follows. Let $O_1$ and $O_2$ be two partitions with $\pi_1=[\ldots,r_1,s_1,\ldots]$ and $\pi_2=[\ldots,r_2,s_2,\ldots]$. Then $O_1 \geq O_2$, while $O_2$ is \emph{not} accessible from $O_1$ if $[\ldots,r_1,s_1,\ldots]=[\ldots,r_2+2k,s_2-2k,\ldots]$ for $k\in \mathbb{Z}_{>0}$, and with $r_1 \geq s_1+6$ and $r_2-2k\neq s_2+2k$.

\textcolor{red}{Create example environment? And find out if TikZ can get to work}The following figure shows the accessibility diagram and the dominance order of nilpotent orbits in $\mathfrak{sp}_8$.
\section{The orthogonal algebras}
\subsection{Partitions and moves}
This section describes some results in the orthogonal algebras. It will show that the matrix forms of nilpotent elements are similar to those in the symplectic algebra, and that the orthogonal moves share similarities with the symplectic moves.

Recall from Section \ref{sec:OrthogonalAlgebra} that the basis of $\mathfrak{o}_n$ is as follows:

\begin{align*}
	\mathcal{B}	&=\{e_1,\ldots, e_n,f_n,\ldots,f_1\} \text{ if Dim}(\mathcal{B})=2n,\\
	\mathcal{B} &=\{e_1,\ldots, e_n,v,f_n,\ldots, f_1\}\text{ if Dim}(\mathcal{B})=2n+1,\\
\end{align*}
and the matrix of the bilinear form with respect to $\mathcal{B}$ is:
$$\Omega_\text{O}=\left(\begin{array}{ccc}
	&  & 1 \\ 
	& \iddots &  \\ 
	1 &  & 
\end{array} \right).$$
Then:
\begin{align*}
	O_n 			&= \{g\in \text{GL}_n \mid g^T \Omega_\text{O} g = \Omega_\text{O}\},\\
	\mathfrak{o}_n	&= \{x \in \mathfrak{gl}_n \mid x^T\Omega_\text{O} +\Omega_\text{O} x = 0 \}.
\end{align*}
Recall the orthogonal case of Theorem \ref{thm:JantzenOrbitsClassicalGroups}:
\begin{theorem*}
	Assume $\phi$ is symmetric (the orthogonal algebra). Then there exists a nilpotent element in $\mathfrak{g}$ with this partition if and only if $r_i$ is even for all even $n_i$.
\end{theorem*}
And Lemma \ref{lem:OrthDistinguished}:
\begin{lemma*}
	Let $x\in \mathfrak{o}_n$, then $x$ is distinguished if and only if its partition $\pi$ has distinct odd parts (and no even parts).
\end{lemma*}
Like in section \ref{SympPartitionsMoves}, here follow the minimal moves through the dominance order of the partitions corresponding to orthogonal nilpotent orbits:
\begin{enumerate}
	\item $\mathcal{O}([2m+1,2m-1])		\rightarrow \mathcal{O}([2m,2m])$.
	\item $\mathcal{O}([2n+1,m,m])		\rightarrow \mathcal{O}([2n-1,m+1,m+1])$.
	\item $\mathcal{O}([n,n,2m-1])		\rightarrow \mathcal{O}([n-1,n-1,2m+1])$.
	\item $\mathcal{O}([n,n,m,m])		\rightarrow \mathcal{O}([n-1,n-1,m+1,m+1])$.
	\item $\mathcal{O}([2n+1,2m+1])		\rightarrow \mathcal{O}([2n-1,2m+3])$.
\end{enumerate}

Comparing with the moves in Section \ref{SympPartitionsMoves}, it shows that the moves in the orthogonal algebra are similar to those in the symplectic algebra; only the sizes of the partitions that occur once are of different size. In moves 2, 3, and 4 there is at most one distinct partition, so there are very similar matrix forms (see Sections \ref{sec:SymplecticAlgebra} and \ref{sec:OrthogonalAlgebra} \textcolor{red}{Find refs} where we determined the standard forms of matrices). Therefore these moves are omitted. In the next section, Move 1 is analysed, because the standard form of a matrix with partition $[2m+1,2m-1]$ is quite different from the standard form of a matrix with partition $[2m,2m-2]$, and it is worth viewing the differences in more detail. Move 5 is impossible to realise with cocharacters, which is analysed in section \ref{Sec:OrthogonalNonMove}. \textcolor{red}{Find Ref}
